Diagonal restriction of Eisenstein series and Kudla-Millson theta lift

We consider the Kudla-Millson theta series associated to a quadratic space of signature $(N,N)$. By combining a `see-saw' argument with the Siegel-Weil formula, we show that its (regularized) integral along a torus attached to a totally real field of degree $N$ is the diagonal restriction of an Eisenstein series. It allows us to express the Fourier coefficients of the diagonal restriction as intersection numbers, which generalizes a result of Darmon-Pozzi-Vonk to totally real fields.

==> todo.tex <==
\section{todo}
\begin{enumerate}
\item check notation of Haar measures
\item make distinction between homology classes and submanifolds $C_\afrak$ and $[C_\afrak]$
\item $G^0$ or $GL2$?, rather $\SL_2$
\item change $g_v=\varsigma_v$? Do i even need?
\item what about genus characters?
\item rename $\id$ by $\Ebf_1$
\end{enumerate}
